Beyond Efficiency: A Systematic Survey of Resource-Efficient Large Language Models

The burgeoning field of Large Language Models (LLMs), exemplified by sophisticated models like OpenAI's ChatGPT, represents a significant advancement in artificial intelligence. These models, however, bring forth substantial challenges in the high consumption of computational, memory, energy, and financial resources, especially in environments with limited resource capabilities. This survey aims to systematically address these challenges by reviewing a broad spectrum of techniques designed to enhance the resource efficiency of LLMs. We categorize methods based on their optimization focus: computational, memory, energy, financial, and network resources and their applicability across various stages of an LLM's lifecycle, including architecture design, pretraining, finetuning, and system design. Additionally, the survey introduces a nuanced categorization of resource efficiency techniques by their specific resource types, which uncovers the intricate relationships and mappings between various resources and corresponding optimization techniques. A standardized set of evaluation metrics and datasets is also presented to facilitate consistent and fair comparisons across different models and techniques. By offering a comprehensive overview of the current sota and identifying open research avenues, this survey serves as a foundational reference for researchers and practitioners, aiding them in developing more sustainable and efficient LLMs in a rapidly evolving landscape.

==> 12-declarations.tex <==
\section{Declarations}



\subsection{Ethics approval and consent to participate}

Not applicable.

\subsection{Consent for publication}

Not applicable.

\subsection{Availability of data and materials}

Data sharing is not applicable to this article as no new datasets were generated or analyzed during the current study. However, this survey discusses and refers to existing datasets that have been duly cited and referenced in Section~\ref{sec: dataset and metrics} of the paper. These datasets are publicly available and have been accessed through their respective repositories or sources, as detailed in the references. Readers are encouraged to refer to these sources for further information on the datasets. For any specific dataset mentioned in Section~\ref{sec: dataset and metrics}, the details about its availability and source are provided in the corresponding citation within the text.


\subsection{Competing interests}

The author(s) declare(s) that they have no competing interests. The authors declare that they have no known competing
financial interests or personal relationships that could have appeared to influence the work reported in this paper


\subsection{Funding}

This work was supported by the National Science Foundation (NSF) under Grant Nos. 1755850, 1841520, 2007716, 2007976, and 1942594; the NSF under Award No. 1907805; a Jeffress Memorial Trust Award; an Amazon Research Award; a NVIDIA GPU Grant; and the Design Knowledge Company (subcontract number: 10827.002.120.04).




\subsection{Authors' contributions}


GB led the project and was responsible for writing the introduction, taxonomy, challenges, future direction, conclusion, and pruning sections.
ZC was responsible for both the system design section and the distributed training part within the pre-training section.
NZ was responsible for the full-parameter fine-tuning within the fine-tuning section and the data efficiency within the pre-training section.
JL was responsible for the architecture design section and the early exit part within the inference section.
SW was responsible for the mixed precision training and quantization within the pre-training and the inference sessions, respectively.
CL was responsible for the parameter-efficient fine-tuning section as well as the knowledge distillation section, respectively.
TS was responsible for the benchmark and evaluation metrics section and for building the GitHub repository.
ZY was responsible for the low-rank approximation section in LLM inference.
MZ and YZ were responsible for the token-parallelism section and for building the GitHub repository.
CY helped substantially revise the paper.
YC proposed the draft for the system design section and helped substantially revise the paper.
LZ was the corresponding author, proposed the idea of the paper, and helped substantially revise the paper.










All authors read and approved the final manuscript.




\subsection{Acknowledgements}

Not applicable.
